Kinetic Langevin MCMC Sampling Without Gradient Lipschitz Continuity -- the Strongly Convex Case

In this article we consider sampling from log concave distributions in Hamiltonian setting, without assuming that the objective gradient is globally Lipschitz. We propose two algorithms based on monotone polygonal (tamed) Euler schemes, to sample from a target measure, and provide non-asymptotic 2-Wasserstein distance bounds between the law of the process of each algorithm and the target measure. Finally, we apply these results to bound the excess risk optimization error of the associated optimization problem.

==> Convex_Hamiltonian <==
@article{momest,
  title={Concentration inequalities for non-Lipschitz functions with bounded derivatives of higher order},
  author={Adamczak, Rados{\l}aw and Wolff, Pawe{\l}},
  journal={Probability Theory and Related Fields},
  volume={162},
  number={3},
  pages={531--586},
  year={2015},
  publisher={Springer}
}

@article{Azagra,
  title={Kirszbraun’s theorem via an explicit formula},
  author={Azagra, Daniel and Le Gruyer, Erwan and Mudarra, Carlos},
  journal={Canadian Mathematical Bulletin},
  volume={64},
  number={1},
  pages={142--153},
  year={2021},
  publisher={Canadian Mathematical Society}
}

@article{Deniz,
  title={Nonasymptotic analysis of Stochastic Gradient Hamiltonian Monte Carlo under local conditions for nonconvex optimization},
  author={Akyildiz, {\"O}mer Deniz and Sabanis, Sotirios},
  journal={arXiv preprint arXiv:2002.05465},
  year={2020}
}

@article{effic6,
  title={Symbolic fenchel conjugation},
  author={Borwein, Jonathan M and Hamilton, Chris H},
  journal={Mathematical Programming},
  volume={116},
  number={1},
  pages={17--35},
  year={2009},
  publisher={Springer}
}

@article{TV,
  title={On explicit $ L\^{} 2$-convergence rate estimate for underdamped Langevin dynamics},
  author={Cao, Yu and Lu, Jianfeng and Wang, Lihan},
  journal={arXiv preprint arXiv:1908.04746},
  year={2019}
}
@article{cheng,
  title={Sharp convergence rates for Langevin dynamics in the nonconvex setting},
  author={Cheng, Xiang and Chatterji, Niladri S and Abbasi-Yadkori, Yasin and Bartlett, Peter L and Jordan, Michael I},
  journal={arXiv preprint arXiv:1805.01648},
  year={2018}
}
@inproceedings{underMCMC,
  title={Underdamped Langevin MCMC: A non-asymptotic analysis},
  author={Cheng, Xiang and Chatterji, Niladri S and Bartlett, Peter L and Jordan, Michael I},
  booktitle={Conference on learning theory},
  pages={300--323},
  year={2018},
  organization={PMLR}
}
@article{Dalaylan,
  title={On sampling from a log-concave density using kinetic Langevin diffusions},
  author={Dalalyan, Arnak S and Riou-Durand, Lionel},
  journal={Bernoulli},
  volume={26},
  number={3},
  pages={1956--1988},
  year={2020},
  publisher={Bernoulli Society for Mathematical Statistics and Probability}
}
@article{newalg,
  title={Explicit formulas for $C^{\{1, 1\}}$ Glaeser-Whitney extensions of 1-Taylor fields in Hilbert spaces},
  author={Daniilidis, Aris and Haddou, Mounir and Le Gruyer, Erwan and Ley, Olivier},
  journal={Proceedings of the American Mathematical Society},
  volume={146},
  number={10},
  pages={4487--4495},
  year={2018}
}
@article{Eberle,
  title={Couplings and quantitative contraction rates for Langevin dynamics},
  author={Eberle, Andreas and Guillin, Arnaud and Zimmer, Raphael},
  journal={The Annals of Probability},
  volume={47},
  number={4},
  pages={1982--2010},
  year={2019},
  publisher={Institute of Mathematical Statistics}
}
@article{Gao,
  title={Breaking reversibility accelerates Langevin dynamics for global non-convex optimization},
  author={Gao, Xuefeng and Gurbuzbalaban, Mert and Zhu, Lingjiong},
  journal={arXiv preprint arXiv:1812.07725},
  year={2018}
}
@incollection{Ledoux,
  title={Concentration of measure and logarithmic Sobolev inequalities},
  author={Ledoux, Michel},
  booktitle={Seminaire de probabilites XXXIII},
  pages={120--216},
  year={1999},
  publisher={Springer}
}
@article{lemarechal1997practical,
  title={Practical aspects of the Moreau--Yosida regularization: Theoretical preliminaries},
  author={Lemar{\'e}chal, Claude and Sagastiz{\'a}bal, Claudia},
  journal={SIAM journal on optimization},
  volume={7},
  number={2},
  pages={367--385},
  year={1997},
  publisher={SIAM}
}
@article{mattingly2002ergodicity,
  title={Ergodicity for SDEs and approximations: locally Lipschitz vector fields and degenerate noise},
  author={Mattingly, Jonathan C and Stuart, Andrew M and Higham, Desmond J},
  journal={Stochastic processes and their applications},
  volume={101},
  number={2},
  pages={185--232},
  year={2002},
  publisher={Elsevier}
}

@article{menz2014poincare,
  title={Poincar{\'e} and logarithmic Sobolev inequalities by decomposition of the energy landscape},
  author={Menz, Georg and Schlichting, Andr{\'e}},
  journal={The Annals of Probability},
  volume={42},
  number={5},
  pages={1809--1884},
  year={2014},
  publisher={Institute of Mathematical Statistics}
}
@book{rockafellar2009variational,
  title={Variational analysis},
  author={Rockafellar, R Tyrrell and Wets, Roger J-B},
  volume={317},
  year={2009},
  publisher={Springer Science \& Business Media}
}
@article{effic18,
  title={Fast Moreau envelope computation I: Numerical algorithms},
  author={Lucet, Yves},
  journal={Numerical Algorithms},
  volume={43},
  number={3},
  pages={235--249},
  year={2006},
  publisher={Springer}
}
@inproceedings{chen2014stochastic,
  title={Stochastic {G}radient {H}amiltonian {M}onte {C}arlo},
  author={Chen, Tianqi and Fox, Emily and Guestrin, Carlos},
  booktitle={International Conference on Machine Learning},
  pages={1683--1691},
  year={2014}
}

@inproceedings{ma2015complete,
  title={A complete recipe for stochastic gradient MCMC},
  author={Ma, Yi-An and Chen, Tianqi and Fox, Emily},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2917--2925},
  year={2015}
}

@article{majka2018non,
  title={Non-asymptotic bounds for sampling algorithms without log-concavity},
  author={Majka, Mateusz B and Mijatovi{\'c}, Aleksandar and Szpruch, Lukasz},
  journal={arXiv preprint arXiv:1808.07105},
  year={2018}
}

@article{gelfand1991recursive,
  title={Recursive stochastic algorithms for global optimization in $\mathbb{R}^d$},
  author={Gelfand, Saul B and Mitter, Sanjoy K},
  journal={SIAM Journal on Control and Optimization},
  volume={29},
  number={5},
  pages={999--1018},
  year={1991},
  publisher={SIAM}
}

@inproceedings{xu2018global,
  title={Global convergence of {L}angevin dynamics based algorithms for nonconvex optimization},
  author={Xu, Pan and Chen, Jinghui and Zou, Difan and Gu, Quanquan},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3122--3133},
  year={2018}
}

@article{dalalyan2019user,
  title={User-friendly guarantees for the {L}angevin {M}onte {C}arlo with inaccurate gradient},
  author={Dalalyan, Arnak S and Karagulyan, Avetik},
  journal={Stochastic Processes and their Applications},
  volume={129},
  number={12},
  pages={5278--5311},
  year={2019},
  publisher={Elsevier}
}


@article{roberts2002langevin,
  title={Langevin diffusions and Metropolis-Hastings algorithms},
  author={Roberts, Gareth O and Stramer, Osnat},
  journal={Methodology and computing in applied probability},
  volume={4},
  number={4},
  pages={337--357},
  year={2002},
  publisher={Springer}
}

@article{dalalyan2017theoretical,
  title={Theoretical guarantees for approximate sampling from smooth and log-concave densities},
  author={Dalalyan, Arnak S},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={79},
  number={3},
  pages={651--676},
  year={2017},
  publisher={Wiley Online Library}
}

@inproceedings{ahn2012bayesian,
  title={Bayesian posterior sampling via stochastic gradient {F}isher scoring},
  author={Ahn, Sungjin and Korattikara, Anoop and Welling, Max},
  booktitle={29th International Conference on Machine Learning, ICML 2012},
  pages={1591--1598},
  year={2012}
}

@article{zhang2019nonasymptotic,
  title={Nonasymptotic estimates for {S}tochastic {G}radient {L}angevin {D}ynamics under local conditions in nonconvex optimization},
  author={Zhang, Ying and Akyildiz, {\"O}mer Deniz and Damoulas, Theodoros and Sabanis, Sotirios},
  journal={Applied Mathematics \& Optimization},
  volume={87},
  number={25},
  year={2023}
}


@article{dalalyan2018sampling,
  title={On sampling from a log-concave density using kinetic {L}angevin diffusions},
  author={Dalalyan, Arnak S and Riou-Durand, Lionel},
  journal={arXiv preprint arXiv:1807.09382},
  year={2018}
}


@article{chau2019fixed,
  title={On fixed gain recursive estimators with discontinuity in the parameters},
  author={Chau, Huy N and Kumar, Chaman and R{\'a}sonyi, Mikl{\'o}s and Sabanis, Sotirios},
  journal={ESAIM: Probability and Statistics},
  volume={23},
  pages={217--244},
  year={2019},
  publisher={EDP Sciences}
}
@article{planiden2019proximal,
  title={Proximal mappings and Moreau envelopes of single-variable convex piecewise cubic functions and multivariable gauge functions},
  author={Planiden, Chayne and Wang, Xianfu},
  journal={arXiv preprint arXiv:1909.05795},
  year={2019}
}

@article{eberle2019couplings,
  title={Couplings and quantitative contraction rates for {L}angevin dynamics},
  author={Eberle, Andreas and Guillin, Arnaud and Zimmer, Raphael},
  journal={The Annals of Probability},
  volume={47},
  number={4},
  pages={1982--2010},
  year={2019},
  publisher={Institute of Mathematical Statistics}
}

@article{chau2019stochastic,
  title={Stochastic {G}radient {H}amiltonian {M}onte {C}arlo for {N}on-{C}onvex {L}earning},
  author={Chau, Huy N and Rasonyi, Miklos},
  journal={arXiv preprint arXiv:1903.10328},
  year={2019}
}

@article{cheng2018sharp,
  title={Sharp convergence rates for {L}angevin dynamics in the nonconvex setting},
  author={Cheng, Xiang and Chatterji, Niladri S and Abbasi-Yadkori, Yasin and Bartlett, Peter L and Jordan, Michael I},
  journal={arXiv preprint arXiv:1805.01648},
  year={2018}
}

@inproceedings{cheng2018underdamped,
  title={Underdamped {L}angevin {MCMC}: {A} non-asymptotic analysis},
  author={Cheng, Xiang and Chatterji, Niladri S and Bartlett, Peter L and Jordan, Michael I},
  booktitle={Conference On Learning Theory},
  pages={300--323},
  year={2018}
}


@article{bubeck2015convex,
  title={Convex optimization: Algorithms and complexity},
  author={Bubeck, S{\'e}bastien and others},
  journal={Foundations and Trends{\textregistered} in Machine Learning},
  volume={8},
  number={3-4},
  pages={231--357},
  year={2015},
  publisher={Now Publishers, Inc.}
}

@inproceedings{raginsky,
  title={Non-convex learning via {S}tochastic {G}radient {L}angevin {D}ynamics: a nonasymptotic analysis},
  author={Raginsky, Maxim and Rakhlin, Alexander and Telgarsky, Matus},
  booktitle={Conference on Learning Theory},
  pages={1674--1703},
  year={2017}
}


@inproceedings{erdogdu2018global,
  title={Global non-convex optimization with discretized diffusions},
  author={Erdogdu, Murat A and Mackey, Lester and Shamir, Ohad},
  booktitle={Advances in Neural Information Processing Systems},
  pages={9671--9680},
  year={2018}
}

@article{durmus2017nonasymptotic,
  title={Nonasymptotic convergence analysis for the unadjusted {L}angevin algorithm},
  author={Durmus, Alain and Moulines, Eric},
  journal={The Annals of Applied Probability},
  volume={27},
  number={3},
  pages={1551--1587},
  year={2017},
  publisher={Institute of Mathematical Statistics}
}

@article{durmus2019high,
  title={High-dimensional {B}ayesian inference via the unadjusted {L}angevin algorithm},
  author={Durmus, Alain and Moulines, Eric},
  journal={Bernoulli},
  volume={25},
  number={4A},
  pages={2854--2882},
  year={2019},
  publisher={Bernoulli Society for Mathematical Statistics and Probability}
}

@article{RobbinsMonro,
  author = {Robbins, H. and Monro, S.},
  journal = {Annals of Mathematical Statistics},
  pages = {400-407},
  title = {A stochastic approximation method},
  volume = 22,
  year = {1951}
}


@phdthesis{ryu2016convex,
  title={Convex optimization for Monte Carlo: Stochastic optimization for importance sampling},
  author={Ryu, Ernest K},
  year={2016},
  school={Stanford University}
}

@article{mei2018landscape,
  title={The landscape of empirical risk for nonconvex losses},
  author={Mei, Song and Bai, Yu and Montanari, Andrea},
  journal={The Annals of Statistics},
  volume={46},
  number={6A},
  pages={2747--2774},
  year={2018},
  publisher={Institute of Mathematical Statistics}
}

@book{nesterov2013introductory,
  title={Introductory lectures on convex optimization: A basic course},
  author={Nesterov, Yurii},
  volume={87},
  year={2013},
  publisher={Springer Science \& Business Media}
}

@techreport{nesterov2011random,
  title={Random gradient-free minimization of convex functions},
  author={Nesterov, Yurii and Spokoiny, Vladimir},
  year={2011},
  institution={Universit{\'e} catholique de Louvain, Center for Operations Research and Econometrics (CORE)}
}


@book{conn2009introduction,
  title={Introduction to derivative-free optimization},
  author={Conn, Andrew R and Scheinberg, Katya and Vicente, Luis N},
  volume={8},
  year={2009},
  series={MPS-SIAM Series on Optimization},
  publisher={SIAM}
}


@article{arouna2004robbins,
  title={Robbins-{M}onro algorithms and variance reduction in finance},
  author={Arouna, Bouhari},
  journal={Journal of Computational Finance},
  volume={7},
  number={2},
  pages={35--62},
  year={2004},
}


@inproceedings{welling2011bayesian,
  title={Bayesian learning via stochastic gradient {L}angevin dynamics},
  author={Welling, Max and Teh, Yee W},
  booktitle={Proceedings of the 28th International Conference on Machine Learning},
  pages={681--688},
  year={2011}
}


@inproceedings{kingma2015adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  booktitle={International Conference on Learning Representations (ICLR)},
  year={2015}
}

@article{kolmogorov1950foundations,
  title={Foundations of the Theory of Probability.},
  author={Kolmogorov, Andrey Nikolaevich},
  year={1950},
  publisher={Chelsea Publishing Co.}
}


@book{doucNLS,
  author = {Randal Douc and Moulines, Eric and Stoffer, David},
  title = {Nonlinear Time Series: Theory, Methods and Applications with R Examples},
  publisher = {Chapman \& Hall},
  year = {2013}
}


@article {MoulinesProximal,
author="Yves F. Atchade and Gersende Fort and Eric Moulines",
title="On stochastic proximal gradient algorithms",
year="2014",
eprint="arXiv/1402.2365",
doi=""
}


@book{bertsekas1999nonlinear,
  title={Nonlinear programming},
  author={Bertsekas, Dimitri P},
  year={1999},
  publisher={Athena scientific}
}

@article{convex,
  title={On stochastic gradient Langevin dynamics with dependent data streams in the logconcave case},
  author={Barkhagen, Mathias and Chau, Ngoc Huy and Moulines, {\'E}ric and R{\'a}sonyi, Mikl{\'o}s and Sabanis, Sotirios and Zhang, Ying},
  journal={Bernoulli},
  volume={27},
  number={1},
  pages={1--33},
  year={2021},
  publisher={Bernoulli Society for Mathematical Statistics and Probability}
}

@inproceedings{brosse2018promises,
  title={The promises and pitfalls of stochastic gradient {L}angevin dynamics},
  author={Brosse, Nicolas and Durmus, Alain and Moulines, Eric},
  booktitle={Advances in Neural Information Processing Systems},
  pages={8268--8278},
  year={2018}
}

@article{tula,
  title={The tamed unadjusted {L}angevin algorithm},
  author={Brosse, Nicolas and Durmus, Alain and Moulines, {\'E}ric and Sabanis, Sotirios},
  journal={Stochastic Processes and their Applications},
  volume={129},
  number={10},
  pages={3638--3663},
  year={2019},
  publisher={Elsevier}
}



@article{nonconvex,
  title={On Stochastic Gradient Langevin Dynamics with Dependent Data Streams: The Fully Nonconvex Case},
  author={Chau, Ngoc Huy and Moulines, {\'E}ric and R{\'a}sonyi, Miklos and Sabanis, Sotirios and Zhang, Ying},
  journal={SIAM Journal on Mathematics of Data Science},
  volume={3},
  number={3},
  pages={959--986},
  year={2021},
  publisher={SIAM}
}

@article{berkeley,
  title={Sharp convergence rates for {L}angevin dynamics in the nonconvex setting},
  author={Cheng, Xiang and Chatterji, Niladri S and Abbasi-Yadkori, Yasin and Bartlett, Peter L and Jordan, Michael I},
  journal={arXiv preprint arXiv:1805.01648},
  year={2018}
}

@article{dalalyan,
  title={Theoretical guarantees for approximate sampling from smooth and log-concave densities},
  author={Dalalyan, Arnak S},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={79},
  number={3},
  pages={651--676},
  year={2017},
  publisher={Wiley Online Library}
}

@article{dk,
  title={User-friendly guarantees for the {L}angevin {M}onte {C}arlo with inaccurate gradient},
  author={Dalalyan, Arnak S and Karagulyan, Avetik},
  journal={Stochastic Processes and their Applications},
  year={2019},
  publisher={Elsevier}
}

@article{unadjusted,
  title={Nonasymptotic convergence analysis for the unadjusted {L}angevin algorithm},
  author={Durmus, Alain and Moulines, Eric and others},
  journal={The Annals of Applied Probability},
  volume={27},
  number={3},
  pages={1551--1587},
  year={2017},
  publisher={Institute of Mathematical Statistics}
}

@article{aew,
  title={High-dimensional {B}ayesian inference via the unadjusted {L}angevin algorithm},
  author={Durmus, Alain and Moulines, Eric and others},
  journal={Bernoulli},
  volume={25},
  number={4A},
  pages={2854--2882},
  year={2019},
  publisher={Bernoulli Society for Mathematical Statistics and Probability}
}

@article{eberleold,
  title={Reflection couplings and contraction rates for diffusions},
  author={Eberle, Andreas},
  journal={Probability theory and related fields},
  volume={166},
  number={3-4},
  pages={851--886},
  year={2016},
  publisher={Springer}
}

@article{Harris,
  title={Quantitative {H}arris-type theorems for diffusions and {M}c{K}ean--{V}lasov processes},
  author={Eberle, Andreas and Guillin, Arnaud and Zimmer, Raphael},
  journal={Transactions of the American Mathematical Society},
  volume={371},
  number={10},
  pages={7135--7173},
  year={2019}
}

@inproceedings{ems,
  title={Global non-convex optimization with discretized diffusions},
  author={Erdogdu, Murat A and Mackey, Lester and Shamir, Ohad},
  booktitle={Advances in Neural Information Processing Systems},
  pages={9671--9680},
  year={2018}
}

@article{hwang,
  title={Laplace's method revisited: weak convergence of probability measures},
  author={Hwang, Chii-Ruey},
  journal={The Annals of Probability},
  volume={8},
  number={6},
  pages={1177--1182},
  year={1980},
  publisher={Institute of Mathematical Statistics}
}



@inproceedings{xu,
  title={Global convergence of {L}angevin dynamics based algorithms for nonconvex optimization},
  author={Xu, Pan and Chen, Jinghui and Zou, Difan and Gu, Quanquan},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3122--3133},
  year={2018}
}

@article{hola,
  title={Higher order {L}angevin {M}onte {C}arlo algorithm},
  author={Sabanis, Sotirios and Zhang, Ying},
  journal={Electronic Journal of Statistics},
  volume={13},
  number={2},
  pages={3805--3850},
  year={2019},
  publisher={The Institute of Mathematical Statistics and the Bernoulli Society}
}



@book{villani2008optimal,
  title={Optimal transport: old and new},
  author={Villani, C{\'e}dric},
  volume={338},
  year={2008},
  publisher={Springer Science \& Business Media}
}

@article{mshloc,
author = {Mattingly, Jonathan and Stuart, A. and Higham, D.},
year = {2002},
pages = {185-232},
title = {Ergodicity for SDEs and approximations: Locally Lipschitz vector fields and degenerate noise},
volume = {101},
journal = {Stochastic Processes and their Applications}
}

@article{chjloc,
author = {Cox, Sonja and Hutzenthaler, Martin and Jentzen, Arnulf},
year = {2013},
journal={arXiv preprint arXiv:1309.5595},
title = {Local Lipschitz continuity in the initial value and strong completeness for nonlinear stochastic differential equations}
}

@article {hutzenthaler2011,
	author = {Hutzenthaler, Martin and Jentzen, Arnulf and Kloeden, Peter E.},
	title = {Strong and weak divergence in finite time of Euler{\textquoteright}s method for stochastic differential equations with non-globally Lipschitz continuous coefficients},
	volume = {467},
	number = {2130},
	pages = {1563--1576},
	year = {2011},
	publisher = {The Royal Society},
	issn = {1364-5021},
	journal = {Proceedings of the Royal Society of London A: Mathematical, Physical and Engineering Sciences}
}

@article{tamed-euler,
author = "Sabanis, Sotirios",
fjournal = "Electronic Communications in Probability",
journal = "Electron. Commun. Probab.",
pages = "1--10",
number = "47",
pno = "47",
publisher = "The Institute of Mathematical Statistics and the Bernoulli Society",
title = "A note on tamed Euler approximations",
volume = "18",
year = "2013"
}

@article{SabanisAoAP,
author = "Sabanis, Sotirios",
fjournal = "The Annals of Applied Probability",
journal = "Ann. Appl. Probab.",
publisher = "The Institute of Mathematical Statistics and the Bernoulli Society",
title = "Euler approximations with varying coefficients: the case of superlinearly growing diffusion coefficients",
volume = "26",
number = "4",
pages = "2083--2105",
year = "2016"
}

@book{hutzenthaler2015numerical,
  title={Numerical approximations of stochastic differential equations with non-globally Lipschitz continuous coefficients},
  author={Hutzenthaler, Martin and Jentzen, Arnulf},
  volume={236},
  number={1112},
  year={2015},
  publisher={American Mathematical Society}
}

@article{hutzenthaler2012,
author = "Hutzenthaler, Martin and Jentzen, Arnulf and Kloeden, Peter E.",
fjournal = "The Annals of Applied Probability",
journal = "Ann. Appl. Probab.",
month = "08",
number = "4",
pages = "1611--1641",
publisher = "The Institute of Mathematical Statistics",
title = "Strong convergence of an explicit numerical method for SDEs with nonglobally Lipschitz continuous coefficients",
volume = "22",
year = "2012"
}

@book{devroye-gyorfi-lugosi,
  title={A probabilistic theory of pattern recognition.},
  author={Devroye, Luc and Gy\"orfi, L\'{a}szl\'{o} and Lugosi, G\'{a}bor},
  year={1996},
  publisher={Springer}
}
@article{TUSLA,
  title={Taming neural networks with TUSLA: Non-convex learning via adaptive stochastic gradient Langevin algorithms},
  author={Lovas, Attila and Lytras, Iosif and R{\'a}sonyi, Mikl{\'o}s and Sabanis, Sotirios},
  journal={To appear, SIAM Journal on Mathematics of Data Science, arXiv:2006.14514},
  year={2020}
}
@article{ovcharova2010second,
  title={Second-order analysis of the Moreau--Yosida and the Lasry--Lions regularizations},
  author={Ovcharova, N},
  journal={Optimization Methods \& Software},
  volume={25},
  number={1},
  pages={109--116},
  year={2010},
  publisher={Taylor \& Francis}
}
@article{tran2018smooth,
  title={A smooth primal-dual optimization framework for nonsmooth composite convex minimization},
  author={Tran-Dinh, Quoc and Fercoq, Olivier and Cevher, Volkan},
  journal={SIAM Journal on Optimization},
  volume={28},
  number={1},
  pages={96--134},
  year={2018},
  publisher={SIAM}
}
@article{boct2020variable,
  title={Variable smoothing for convex optimization problems using stochastic gradients},
  author={Bo{\c{t}}, Radu Ioan and B{\"o}hm, Axel},
  journal={Journal of Scientific Computing},
  volume={85},
  number={2},
  pages={1--29},
  year={2020},
  publisher={Springer}
}

@article{durmus2018efficient,
  title={Efficient bayesian computation by proximal markov chain monte carlo: when langevin meets moreau},
  author={Durmus, Alain and Moulines, Eric and Pereyra, Marcelo},
  journal={SIAM Journal on Imaging Sciences},
  volume={11},
  number={1},
  pages={473--506},
  year={2018},
  publisher={SIAM}
}
@book{vershynin2018high,
  title={High-dimensional probability: An introduction with applications in data science},
  author={Vershynin, Roman},
  volume={47},
  year={2018},
  publisher={Cambridge university press}
}
@article{otto2000generalization,
  title={Generalization of an inequality by Talagrand and links with the logarithmic Sobolev inequality},
  author={Otto, Felix and Villani, C{\'e}dric},
  journal={Journal of Functional Analysis},
  volume={173},
  number={2},
  pages={361--400},
  year={2000},
  publisher={Elsevier}
}
@article{johnston2021strongly,
  title={A Strongly Monotonic Polygonal Euler Scheme},
  author={Johnston, Tim and Sabanis, Sotirios},
  journal={arXiv preprint arXiv:2112.15596},
  year={2021}
}
@article{zhang2020first,
  title={First-Order Algorithms Without Lipschitz Gradient: A Sequential Local Optimization Approach},
  author={Zhang, Junyu and Hong, Mingyi},
  journal={arXiv preprint arXiv:2010.03194},
  year={2020}
}
@article{gao2021global,
  title={Global Convergence of Stochastic Gradient Hamiltonian Monte Carlo for Nonconvex Stochastic Optimization: Nonasymptotic Performance Bounds and Momentum-Based Acceleration},
  author={Gao, Xuefeng and G{\"u}rb{\"u}zbalaban, Mert and Zhu, Lingjiong},
  journal={Operations Research},
  year={2021},
  publisher={INFORMS}
}
@article{harge2004convex,
  title={A convex/log-concave correlation inequality for Gaussian measure and an application to abstract Wiener spaces},
  author={Harg{\'e}, Gilles},
  journal={Probability theory and related fields},
  volume={130},
  number={3},
  pages={415--440},
  year={2004},
  publisher={Springer}
}

